A Large Scale Analysis of Android-Web Hybridization

Many Android applications embed webpages via WebView components and execute JavaScript code within Android. Hybrid applications leverage dedicated APIs to load a resource and render it in a WebView. Furthermore, Android objects can be shared with the JavaScript world. However, bridging the interfaces of the Android and JavaScript world might also incur severe security threats: Potentially untrusted webpages and their JavaScript might interfere with the Android environment and its access to native features. No general analysis is currently available to assess the implications of such hybrid apps bridging the two worlds. To understand the semantics and effects of hybrid apps, we perform a large-scale study on the usage of the hybridization APIs in the wild. We analyze and categorize the parameters to hybridization APIs for 7,500 randomly selected and the 196 most popular applications from the Google Playstore as well as 1000 malware samples. Our results advance the general understanding of hybrid applications, as well as implications for potential program analyses, and the current security situation: We discovered thousands of flows of sensitive data from Android to JavaScript, the vast majority of which could flow to potentially untrustworthy code. Our analysis identified numerous web pages embedding vulnerabilities, which we exemplarily exploited. Additionally, we discovered a multitude of applications in which potentially untrusted JavaScript code may interfere with (trusted) Android objects, both in benign and malign applications.

==> sections/loadurl-semantics.tex <==
\newcommand{\WebView}{\emph{WebView}~}

\subsubsection{Semantics of communication between Android Java and Javascript}
Android provides two ways of communication between Java and javascript: (1)
Callback communication and (2) Bridge communication.~\cite{lee2016hybridroid}.

\paragraph*{Callback Communication} Android SDK defines callback
methods in the class \emph{WebChromeClient} and
\emph{WebViewClient}. These methods are triggered by specific events in
\emph{WebView}. For example a method \emph{onPageFinished(WebView wv, String
url)} is triggered when a page loading is completed.

\paragraph*{Bridge Communication} Android allows to annotate certain methods 
with \texttt{JavascriptInterface}. These methods can be later called in the 
\emph{loadUrl} either directly using the annotation \textit{javascript} or in some javascript defined in 
the target URL in \emph{loadUrl}. Listing~\cite{listing:MainActivity1}
shows one example of Bridge communication.

